Adaptive Path Planning for UAV-based Multi-Resolution Semantic Segmentation

In this paper, we address the problem of adaptive path planning for accurate semantic segmentation of terrain using unmanned aerial vehicles (UAVs). The usage of UAVs for terrain monitoring and remote sensing is rapidly gaining momentum due to their high mobility, low cost, and flexible deployment. However, a key challenge is planning missions to maximize the value of acquired data in large environments given flight time limitations. To address this, we propose an online planning algorithm which adapts the UAV paths to obtain high-resolution semantic segmentations necessary in areas on the terrain with fine details as they are detected in incoming images. This enables us to perform close inspections at low altitudes only where required, without wasting energy on exhaustive mapping at maximum resolution. A key feature of our approach is a new accuracy model for deep learning-based architectures that captures the relationship between UAV altitude and semantic segmentation accuracy. We evaluate our approach on the application of crop/weed segmentation in precision agriculture using real-world field data.

==> aux.tex <==
\section{aux}
Our idea is to use the semantic information to infer which regions of the field require to be mapped with higher resolution.
We assume that the accuracy is increasing with a higher resolution and infer: The more interesting it is, the more time it is worth to take some more images with a higher resolution from a lower altitude. The more intelligent the desired resolution is chosen, the more the trade-off between high accuracy and a low execution time turns out to be in our favor. 
We quantify the level of interest by the vegetation ratio:\\
\begin{equation}\label{eq:ratio}
ratio = \dfrac{\# crop + \# weed}{\# crop + \# weed + \# background}
\end{equation}
Each pixel is segmented as crop, weed, or background. If the field section consists to a large extent of vegetation pixels (crop+weed), the section is planted more densely, contains a larger amount of information, and thus contains more potential for higher accuracy through an additional recording with a higher resolution than a sparsely planted field section. Therefore, we capture the vegetation ratio as criteria and introduce a decision function to map the ratio to a desired resolution. Then, the current waypoint is taken with the calculated resolution, before the overall flight path is being continued. A higher resolution is synonymous with a lower altitude and a smaller footprint. More than one image from a lower altitude is needed to cover the same area like was covered from the high altitude. The flight path for one waypoint is again a lawn mower strategy, consisting of single subordinate waypoints.

One simple approach to use the segmentation in the form of the vegetation ratio is to map the ratio linearly to the resolution. More precisely, the resolution is then minimal if the ratio is smaller than a defined minimum ratio value, maximal if the ratio is higher than a defined maximum ratio value, and mapped linearly to a resolution if the ratio lies in the range between these border values. A decision function with linear mapping is subject to the simplified assumption that the segmentation accuracy is increasing linearly with the resolution. In this case, it would be assumed that a certain increase in resolution always results in a certain increase in accuracy, regardless of the resolution itself. 

We overcome the need of making any assumption and refine the shape of the decision function based on the incoming observations. The informative path planning strategy uses previous runs on a separate field as prior knowledge for initialization and uses new incoming observations to update the function shape online. 

We initialize the shape of the decision function within the range where the function is non-constant.
The range has to be specified and fixes the function on the x-axis. A minimum altitude for the waypoints with the highest resolution requirement has to be specified as well and fixes the function on the y-axis. The ranges are fixed during the flight, whereas the shape of the function is data-adaptive. 
The decision function is initialized in advance. We use a separate field for initialization to already start the flight with some previous knowledge and with a decision function shape, which is data-based.

The initialization is carried out to gain some knowledge about how the accuracy relates to the resolution. The separate field is mapped and segmented with different single resolutions. Then, the segmentation accuracy is computed by comparison with the ground truth and saved for each run. The respective accuracy, related to the accuracy for the lowest resolution, provides the respective accuracy gain to cover the field with a correspondingly higher resolution. Multiple resolution settings result in multiple points, arranged in a shape that we make use of. We mirror the plots on the $x$-axis and thus follow the idea to translate a high positive derivative to a correspondingly high negative derivative. It means, that we are more willing to increase the resolution in an area in which the accuracy increases more with the resolution, just because we expect a higher increase in accuracy from an increase in resolution there. In the following, the obtained points are scaled and set into the defined range. The points are then fitted by using the \textit{Gaussian Process Regression} (see \ref{subsec:update}). Figure \ref{fig:initialization} shows the initialization pipeline, which results in the initialized decision function with its data-adaptive shape.
We discretize this function into a step function in the last step, because the number of images that are needed for covering the area of a high altitude-footprint from lower altitude does also increase in steps with a lower altitude. The resolutions to which the values are discretized are chosen so, that the ratio between the resolution and the number of images is optimal.\\

Besides the initialization of the decision function shape, we also initialize a regression function between the vegetation ratio and the accuracy. We save not only the accuracy gain for multiple resolution differences on the separate field used for initialization but also the respective vegetation ratio. Thus, we receive additional information about the relation of the accuracy gain with respect to the vegetation ratio gain. The accuracy is the objective that we want to maximize and does therefore also serve to specify the function shape. But the accuracy can only be computed after the field segmentation has been completed. This would collide with our claim to adapt the shape during the flight based on the observations, so we use the vegetation ratio gain as online available information. It enables indirect access to the respective accuracy gain with an increased resolution. Using the ratio gain directly for evaluating the worth of having gone down, would neglect the fact that a higher ratio could also mean a higher number of \textit{False Positives}. That would only be a reasonable approach if the assumption holds, that a higher ratio leads in any case to higher accuracy. We use a polynomial approximation of the accuracy for a given ratio as regression. Based on the observation we choose a 4th-degree polynomial:

\begin{equation}\label{eq:polynomial}
p(x) = ax^4 + bx^3 + cx^2 + dx + e
\end{equation}

The resulting fitted polynomial with parameters $a$-$e$ minimizes the squared error $E$ between the polynomial points $p(x_j)$ and the observations $y_j$ for $k$ points:

\begin{equation}\label{eq:kq}
E = \sum_{j=0}^k |p(x_j)-y_j|^2
\end{equation}

The polynomial parameters are valid over the entire flight. The mapping from the ratio gain to the accuracy gain stays constant and is therefore based exclusively on the data from the separate field.\\


Figure \ref{fig:workflow} shows the procedure for one waypoint from the preliminary flight path. After extracting and segmenting a footprint, the vegetation ratio is calculated and mapped to a \textit{Ground Sampling Distance} (GSD) with which another footprint is extract and segmented. The mapping is done via the initialized decision function or the updated one if the decision function has already been updated. The segmentation with higher resolution is preferred if the resolution gain has led to an accuracy gain. For evaluating this, the ratio gain between the two vegetation ratios is calculated and mapped to the accuracy gain. If the accuracy gain is positive, the segmentation with higher resolution seems to be more accurate and is therefore used for the total field segmentation. We used the information obtained in this procedure to adapt the shape of the decision function online.

\begin{figure}[t]
 \centering
 \includegraphics[width=0.75\linewidth]{pics/Fig2_new}
 \caption{The initialized decision function in comparison with the baseslines. The function is no langer constant or linear in the active range. The function shape comes from the initialization on a separate field and will be updated online.}
 \label{fig:linmapfunc}
\end{figure}


\subsection{Online shaping of the decision function}
\label{subsec:update}

The initialization was carried out on another field whose characteristics represent the characteristics of the current field only approximatively. Including experience which has already been gained during the flight over the current field adapts the shape of the decision function update by update more closely to the current field's characteristic. In addition to the mentioned functionality as a decision criterium, the accuracy gain is also the basis for updating the decision function. Taking a segmentation for a footprint with two different resolutions provides two pieces of information that can be used for updating:

\begin{itemize}
 \item GSD difference: Higher GSD minus Lower GSD
 \item Ratio difference: Ratio for an image with higher GSD minus Ratio for an image with lower GSD
\end{itemize} 

The ratio difference is mapped to the accuracy gain via the fixed regression function. The accuracy gain for a given resolution difference means a new observation, which is included for fitting the decision function shape. Every time a viewpoint is recorded with two different resolutions, the procedure is carried out. The decision function is re-fitted and gets a new shape.  

The observations are fitted via a \textit{Gaussian Process Regression}. The \textit{Gaussian Process Regression} is a Bayesian non-parametric approach and therefore not limited by any functional form.
We have present observations as $X$ ($x$-values) and $y$ (corresponding $y$-values). Then, we specify a Gaussian Prior $p(w)$ and apply \textit{Bayes' Rule} for getting the posterior distribution: 

\begin{equation}\label{eq:bayes}
p(w|y,X) = \frac{p(y|X,w)p(w)}{p(y|X)}
\end{equation}

$p(y|X,w)$ is the \textit{likelihood}, $p(y|X)$ the \textit{marginal likelihood}. For a new incoming observation $x^{*}$, we calculate the predictive distribution $f^{*}$, which is the corresponding $y$-value:

\begin{equation}\label{eq:predictive}
p(f^{*}|x^{*},y,X) = \int_w p(f^{*}|x^{*},w)p(w|y,X)
\end{equation}

We can rewrite the \textit{Gaussian Prior} to: 


The \textit{Gaussian Process} is completely defined by the mean function $m(x)$ and the covariance function/kernel $k(x,x')$. The kernel specifies the statistical relationship between two points $x$ and $x'$. We specify the \textit{Prior} by specifying the kernel and use a constant kernel and an \textit{Radial Basis Function} kernel. Together, we get the following kernel function: 

\begin{equation}\label{eq:kernel}
k(x,x') = \sigma_{f}^{2} exp(-\frac{1}{2\ell^{2}}||x-x'||^{2})
\end{equation}

The kernel has two hyperparameters, the \textit{signal variance} $\sigma_{f}^{2}$ and the \textit{lengthscale} $\ell$. The signal variance is set via an alpha parameter to $0.2$, so each observation is considered to be trustworthy. We use a length scale of $1.0$ and lengthscale bounds $1e-6$ and $1e1$ for the constant kernel and a a lengthscale of $0.01$ and lengthscale bounds of $1e-6$ and $1e-1$ for the \textit{RBF} kernel. Especially, the situation of identical values is very common when using a step function and favors the use of a \textit{Gaussian Process Regression} over a parametric approach.



\subsection{Baselines}
\label{subsec:baselines_aux} 


The single-resolution lawn-mower strategy from the defined maximum resolution and the defined minimum resolution, as well as the linear decision function, work as baselines. The maximum and minimum resolution mappings work as upper and lower bound, which interpret the trade-off of maximizing the accuracy while minimizing the execution time completely in favor of one and at the expense of the other criterion. Our multi-resolution approach gets values in between, striving towards the accuracy of the high resolution and the low time of the low resolution as far as possible. The linear decision function works as the relevant baseline. Performing better than this multi-resolution approach shows that our approach can reach better results by shaping the decision function based on the gained data knowledge.

We quantify the accuracy by the \textit{Intersection over Union} ($IoU$) metric. The $IoU$ is defined as the number of overlapping pixels divided by the number of union pixels. The metric can be computed for each class, but we do not differentiate between the single classes and take the mean $IoU$ as the representative value for the accuracy term, which is to be maximized.

The execution time consists of the time the drone needs to fly from waypoint to waypoint and of the time the drone needs to take the image at one waypoint. A UAV Controller is implemented from \cite{sakai2019}. It is implemented in $SO(3)$ to take the three-dimensional drone kinematics into account. The execution time can be obtained by taking the time for following the trajectory defined by the waypoints. For our application, there is no change in drone orientation needed, and there are only linear trajectory sequences with zero start and end velocities. To this, we do not take any uncertainties into account. For this case it simplifies to a sequence of linear trajectories for which the respective execution time can be computed with the given path length, a predefined maximum drone velocity $v_{max}$, and a predefined maximum drone acceleration $a_{max}$ via the \textit{Trapezoids Law}. The law enforces a linear increase in velocity at the beginning, a linear decrease in velocity at the end, and a constant velocity in between. This way, the execution time can be calculated unambiguously also for images without georeferenced coordinates.\\
The execution time is calculated with $v_{max}=5m/s$ and $a_{max}=2m/s^2$, where the absolute values are less interesting than the relative execution time differences.
In the end, a constant amount of time for each waypoint is added manually for taking the images. The constant time is set to $5s$ per waypoint, so the product of this duration and the number of images is added. The two-dimensional view of the results brings with it the problem of comparability. Besides, the decision functions – the advanced one as well as the linear one - have no fixed defined $x$- range.

\subsection{Results}
\label{sec:results_aux}

The performance is evaluated with initialization at field $03$ and an application on field $00$ and $02$.
Figure \ref{fig:results2} shows the averaged performances for the testing fields. 
The various results obtained with a linear decision function give information about the trade-off. They show, that an increase in accuracy generally has to be paid for with a larger time requirement, and vice versa. This relation is approximately linear and about a 1\% higher $IoU$ per $500s$.


 
We can show that our approach can not only improve the trade-off compared to the linear decision function but that in some cases we even get an increase in accuracy with greatly reduced execution time. It means, that we can achieve two strongly conflicting goals at the same time, so we invest the additional time for getting higher resolution more efficiently than a less data-adaptive approach. \\
Figure \ref{fig:waypoints} shows the different flight paths for the respective strategies. In our approach, the drone is selective in going down to a certain altitude and the resulting path length is visibly shorter than in the linear baseline approach.
Figure \ref{fig:results2} shows two scenes where our approach performs better than the baseline. While the linear decision function does not notice the need for a higher resolution and outputs a higher GSD, the adaptive decision function notices that here a higher resolution is worthwhile to better capture the plants and to get higher accuracy. 

Note that not only the performance for a linear mapping function but also the performance for the advanced strategy depends on the range of the non-constant mapping function. Start and range of this range are further parameters that should also be taken from the field for initialization. Because this work focuses on the shape of the decision function, the used ranges have not been selected according to a completely defined scheme.

The used fields have a quite homogeneous crop and weed distribution in large parts. It is expected that a less homogeneous distribution would further increase the gain of our approach and realize the potential of this approach even better.



